Hardware-Aware Automated Neural Minimization for Printed Multilayer Perceptrons

The demand of many application domains for flexibility, stretchability, and porosity cannot be typically met by the silicon VLSI technologies. Printed Electronics (PE) has been introduced as a candidate solution that can satisfy those requirements and enable the integration of smart devices on consumer goods at ultra low-cost enabling also in situ and ondemand fabrication. However, the large features sizes in PE constraint those efforts and prohibit the design of complex ML circuits due to area and power limitations. Though, classification is mainly the core task in printed applications. In this work, we examine, for the first time, the impact of neural minimization techniques, in conjunction with bespoke circuit implementations, on the area-efficiency of printed Multilayer Perceptron classifiers. Results show that for up to 5% accuracy loss up to 8x area reduction can be achieved.

==> Sections/old_sections/background_2.tex <==
\section{Background}

\AK{ mia sthlh max }

==> Sections/old_sections/conclusions_5.tex <==
\section{Conclusions}
Printed electronics is a promising solution to bring ``intelligence'' in application domains characterized by ultra-low-cost fabrication and flexibility requirements.
In this paper, we present a co-design methodology for printed MLPs.
Our hardware-aware neural minimization, combined with fully customized circuit implementations, delivers very high hardware gains ($4$x on average) even at zero accuracy loss.
Importantly, for only 5\% loss, our co-design enables, for the first time, battery-powered operation of complex printed MLPs.

==> Sections/old_sections/evaluation_4.tex <==
%\begin{figure}[t!]
%\centering
%\begin{subfigure}{.48\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{Figures/scatter_ww_rw.png} 
%\end{subfigure}
%\begin{subfigure}{.48\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{Figures/cardio_vertebral_scatter.png}  
%\end{subfigure}

%\begin{subfigure}{.48\textwidth}
%   \centering
%    \includegraphics[width=\textwidth]{Figures/scatter_pendigits_seeds.png}  
%\end{subfigure}
%\caption{True Pareto fronts after synthesis and gate-level simulation showing normalized power %consumption Vs accuracy for three standalone approximation techniques and our framework's at 1V. %Examined MLP classifiers: (a) White-wine, (b) Red-wine, (c) Cardio (d) Vertebral, (e) Pendigits, (f) %Seeds.}
%\label{fig:scatter_plots}
%\end{figure}

\begin{figure}[t!]
\centering
    \centering
    \includegraphics[width=\columnwidth]{Figures/scatter_plots.PDF} 
\caption{Area-Accuracy trade-off of the printed MLPs produced by our framework, only pruning, only quantization, and only weight sharing. Values are normalized over each baseline MLP~\cite{Mubarik:MICRO:2020:printedml}.
MLP classifiers: (a) WhiteWine, (b) RedWine, (c) Cardio (d) Vertebral (3C), (e) Pendigits, (f) Seeds.}
\label{fig:scatter_plots}
  \vspace{-.2in}
\end{figure}


\section{Results and Analysis}\label{sec:eval}

In this section, we evaluate the efficiency of our framework in generating area- and power- efficient printed MLPs and assess its effectiveness in enabling their battery powered operation.
To that end, we consider six classification MLPs trained on the  RedWine, WhiteWine, Cardiotocography, Vertebral (3 column), Pendigits, and Seed datasets of the UCI ML repository~\cite{Dua:2019:uci}, similarly to~\cite{Armeniakos:DATE2022:axml,Weller:2021:printed_stoch}.
Synopsys Design Compiler and PrimeTime are used for synthesis and power analysis, respectively, while QuestSim is used for circuit simulation.
The open source Electrolyte Gated Transistor (EGT)--an inkjet-printed technology-- library~\cite{Bleier:ISCA:2020:printedmicro} is used.
The delay constraint for Pendigits is 250ms and for the rest MLPs 200ms.
Since we consider fully parallel architectures, this is also the latency of a single inference.
Such values are in alignment with typical performance of printed electronics~\cite{Bleier:ISCA:2020:printedmicro} and they are almost identical with the inference latency reported in the respective state-of-the-art~\cite{Armeniakos:DATE2022:axml,Weller:2021:printed_stoch}.
In our genetic algorithm we set the population size to 40 and the number of generations to 50. 

First, we evaluate the area-efficiency of the MLPs produced by our co-design methodology.
As baseline printed MLPs we consider the un-simplified bespoke implementation~\cite{Mubarik:MICRO:2020:printedml} of the models obtained from NAS.
Fig.~\ref{fig:scatter_plots} presents the area-accuracy of our printed MLPs.
The values are normalized w.r.t. the area and accuracy of the respective baseline.
The voltage value is set to $1$V for all the designs in Fig.~\ref{fig:scatter_plots}.
Similar results are obtained for power-accuracy but are not presented here due to space limitation.
Moreover, Fig.~\ref{fig:scatter_plots} depicts the same analysis for each technique when applied in isolation, i.e., bespoke MLP circuits with only quantization, pruning, or weight sharing.
Compared to the baseline~\cite{Mubarik:MICRO:2020:printedml}, our MLPs feature very high area reduction for minimal accuracy loss.
Indicatively, on average, our MLPs exhibit $4.1$x less area than the baseline~\cite{Mubarik:MICRO:2020:printedml} for no accuracy loss.
Furthermore, our MLPs constitute the most efficient solutions as they always appear on the Pareto-front in Fig.~\ref{fig:scatter_plots}.
Specifically, for similar accuracy, our MLPs achieve on average $3.2$x, $3.6$x, and $23$\% lower area compared to only weight sharing, pruning, and quantization, respectively.
Interestingly, Seeds is highly amenable to low-precision and thus, many of the designs produced by our framework apply only quantization, featuring more than $2.4$x area reduction.
For Vertebral, our framework found a solution in which almost all weights feature zero-area (e.g., powers-of-2) or are shared.
For no accuracy loss, only 6 out of 27 multipliers are instantiated.
%At this point we must note that the voltage value is set to $1$V for all the designs of Fig~\ref{fig:scatter_plots}.
%The main reason of using $1$V for all the designs is to simplify the comparisons and deliver a straightforward comparison.
%The baseline assumes $1$V while only pruning doesn't always result in a delay gain requiring also $1$V operation.

\begin{figure}[t!]
\centering
    \centering
    \includegraphics[width=\columnwidth]{Figures/Fig5.PDF} 
\caption{a) Area and b) power reduction achieved by our printed MLPs compared to the state-of-the-art approximate~\cite{Armeniakos:DATE2022:axml} and stochastic~\cite{Weller:2021:printed_stoch} ones.
Iso-accuracy evaluation is considered.}
\label{fig:soa}
  \vspace{-.2in}
\end{figure}

Next, in Fig.~\ref{fig:soa}, we compare our MLPs against the current state-of-the-art~\cite{Armeniakos:DATE2022:axml,Weller:2021:printed_stoch} that also consider complex printed MLP classifiers.
In~\cite{Armeniakos:DATE2022:axml} and~\cite{Weller:2021:printed_stoch}  approximate and stochastic computing are employed, respectively.
In Fig.~\ref{fig:soa} we consider an iso-accuracy evaluation.
When comparing our MLPs with~\cite{Armeniakos:DATE2022:axml} we set the accuracy threshold to $1$\% for both frameworks. 
When comparing against~\cite{Weller:2021:printed_stoch} we set the accuracy threshold for our MLPs equal to the accuracy achieved by the respective stochastic MLP of~\cite{Weller:2021:printed_stoch}.
Since~\cite{Armeniakos:DATE2022:axml,Weller:2021:printed_stoch} consider high voltage operation, we again set (as in Fig.~\ref{fig:scatter_plots}) the voltage value of our circuits to $1$V. 
As shown in Fig.~\ref{fig:soa}, our MLPs outperform significantly both the approximate~\cite{Armeniakos:DATE2022:axml} and the stochastic~\cite{Weller:2021:printed_stoch} MLPs.
Compared to~\cite{Armeniakos:DATE2022:axml}, our MLPs feature on average $3.3$x and $3$x lower area and power, respectively.
Similarly, compared to~\cite{Weller:2021:printed_stoch}, our MLPs achieve $3.2$x and $3.4$x lower area and power.


\input{Sections/tab_battery}

Furthermore, we assess the effectiveness of our framework in generating battery powered printed MLPs.
Unlike Fig.~\ref{fig:scatter_plots} and~\ref{fig:soa}, in this evaluation we employ the full-potential of our framework by also applying voltage scaling.
We consider two accuracy loss constraints, i.e., $1$\% and $5$\%, and present in Table~\ref{tab:battery} the accuracy and hardware characteristics of our MLPs that feature the least power consumption and satisfy the accuracy constraint.
The circuits are synthesized at a reduced voltage value and thus, at the same accuracy, the designs in Table~\ref{tab:battery} might be different than the ones in Fig.~\ref{fig:scatter_plots} or there might be some slight area differences for the same designs.
As shown in Table~\ref{tab:battery}, for $1$\% accuracy loss, our MLPs achieve $19$x lower power consumption on average than the baseline MLPs.
For $5$\% accuracy loss, the average power gain increases to $32.7$x.
Similarly, the area gain is on average $6.2$x and $12.4$x for the $1$\% and $5$\% loss thresholds.
In the Vertebral MLP for no accuracy loss we achieve $12.6$x and $2.6$x power and area gains respectively.
Moreover, as shown in Table~\ref{tab:battery}, for all the MLPs (except from Pendigits) a voltage value of $0.6$V is selected by our voltage scaling. 
In other words, the delay gain due to our neural minimization enabled almost all the MLPs to operate at the lowest voltage value without any performance loss.
Note that the baseline MLPs cannot meet the delay constraint below $1$V.
In Table~\ref{tab:battery}, we use a color code to represent the batteries that could power our MLPs.
Orange represents a Molex $30$mW batery, light blue a Zinergy $15$mW, dark blue a BlueSpark $3$mW, green a printed energy harvester, while no color means that there is no adequate power supply.
As shown, for $5$\% accuracy loss all our MLPs can be battery-powered while for $1$\% loss only Pendigits cannot.
Moreover, RedWine and Seeds can even be powered by an energy harvester.
Note that none of the respective baseline MLPs can be battery-powered.
To the best of our knowledge, this is the first time that such complex printed ML circuits can be battery-operated.
Indicatively, Pendigits features 15 neurons and $130$ weights.
Finally, all our MLPs feature mainly a reasonable area to be considered for a printed application. 

Finally, we evaluate the time-efficiency of our framework and the accuracy of our area estimator.
Our framework's exploration time is on average 140 min ranging from 38 min to 260 min.
These values refer to a single-threaded execution on a Xeon 5218R server.
A parallel chromosome evaluation in the \mbox{NSGA-II} can minimize these times.
To assess the accuracy of our area estimator, we randomly generated $5,000$ MLPs and evaluated their area.
The $R^2$ score of our area estimator is $0.75$.
Most importantly, its Pearson correlation coefficient is $0.89$, i.e., very good linear correlation.
Hence, our estimator can predict with high confidence if a MLP is more area efficient than another one and, thus, is perfectly capable in guiding our optimization search towards more area-efficient solutions. 


%ranges from 38 min to 260 min, for the Vertebral and the WhiteWine respectively, with an average exploration time of 140 min.
% We evaluate the accuracy of our area estimator using 1,000 randomly generated printed MLPs.
% The $R^2$ score of our area estimator is $0.75$.
% Most importantly, its Pearson correlation coefficient is $0.89$, i.e., very good linear correlation.
% Hence, our estimator can predict with high confidence if a MLP is more area efficient than another one and guide our optimization search (see Section~\ref{sec:framework}) towards more efficient solutions. 


==> Sections/old_sections/evaluation_4_aG.tex <==
\section{Results and Evaluation}
In this section the evaluation analysis of the proposed framework is presented where we investigate the framework's efficiency to generate low-power and low-area designs for six different classifiers.
Specifically, we examine models trained on the RedWine, WhiteWine, Cardiotocography, Vertebral, Pendigits and Seed datasets of the UCI ML repository~\cite{} following the RTL realization that is described in subsection~\ref{synthesis}.
The examined circuits are synthesized at a timing constraint of 200 \textit{ms}, besides the Pendigits classifier that is synthesized at 250 \textit{ms}.
For every evaluated classifier the framework's NSGA-II genetic optimization algorithm was set to halt after 40 generations with 40 candidate chromosomes being evaluated for their inference error and their area overhead at each generation.
The algorithm's output is the estimated Pareto area-accuracy front that is produced by the final population.

First we compare our framework's holistic approach with the standalone approximation techniques.
This analysis is presented in Figure\ref{scatter_plots}. The presented Paretos were generated for the examined datasets when: \textbf{(a)} our proposed framework is enabled for number of clusters \(M\)  between two to 9 (red '\(\largestar\)'),
\textbf{(b)} only quantization is applied (green '\( \bigcirc\)' ), \textbf{(c)} only pruning with sparsity range between 10\% to 80\% is applied (yellow '\(\bigtriangledown\)'  ) and \textbf{(d)} only the weight clustering approach~\cite{sharing:ICLR2016} for number of clusters (\(M\)) between two to 9 is used (blue '\( \bigtriangleup \)'). In all cases the hardware friendly RTL realization that is described in subsection \ref{synthesis} was followed. For the \textbf{(c)} and \textbf{(d)} evaluation scenarios, an 8-bit representation for the weights and the biases; and a 4-bit representation for the network's inputs was selected.
Noted that for the Pareto points that are identical with those generated from our framework only the latter ones are depicted. 
Figure~\ref{scatter_plots} presents the true power consumption-accuracy Paretos after synthesis and gate-level simulation of our framework's estimated Paretos for the examined datasets at 1V. 
Power consumption and accuracy are presented normalized w.r.t the values of the our baseline~\cite{Mubarik:MICRO:2020:printedml} models. Noted that the area-accuracy Pareto points are identical and therefore they are not presented in the scope of this analysis.

Overall, our framework generates more power and area efficient designs compared to the solutions that are produced from the standalone approximations; this is due to the employment of multiply approximation techniques that are combined together leading to higher gains.
It is observed that most of the Pareto fronts are composed of a few dominant designs. In the cardio classifier (i.e Figure~\ref{fig:scatter_plotsscatter_plots}c) there is one optimal design that employs the only quantization technique.
In the specific dataset a 2-bit representation of the network's weights is adequate for achieving the accuracy of the baseline network.
On the other hand, in the seeds classifier (i.e Figure~\ref{fig:scatter_plotsscatter_plots}f) the Pareto front of the only quantized designs is a subset of our framework's Paretos.
Looking at the redwine and vertebral classifiers (Figures \ref{fig:scatter_plots}b and \ref{fig:scatter_plots}d) there are Pareto solution that achieve higher accuracy from the baseline models. This may happen~\cite{} due to the QA retraining that our framework's perform to fine-tune the values of the quantized coefficients.

Next, we compare our framework's results with two state-of-the-art methodologies that leverage bespoke approximation~\cite{Armeniakos:DATE2022:axml} and stochastic techniques~\cite{Weller:2021:printed_stoch}. The comparisons with the manuscript's~\cite{Armeniakos:DATE2022:axml} classifiers were performed between designs that have an up to 1\% accuracy degradation from the baseline~\cite{Mubarik:MICRO:2020:printedml} networks, while for the stochastic approach iso-accuracy designs are compared. The results of this evaluation analysis are shown on Figure~\ref{fig:barplots}.
It is observed that our framework generates designs that are on average 3.2x and 3.75x more area and power efficient respectively compared to the bespoke approximate classifiers~\cite{Armeniakos:DATE2022:axml} for the same accuracy loss.
Similarly, compared to the stochastic classifiers~\cite{Weller:2021:printed_stoch} our framework leads to an average increase by 1.95x and 2.43x at the circuits' area and power gains for similar classification accuracy.

Finally, Table~\ref{tab:table_platforms} presents the gains of the power optimal classifiers for 1\% and 5\% accuracy loss from our baseline networks~\cite{Bleier:ISCA:2020:printedmicro}.
Those networks are generated after the voltage scaling optimization step. We highlight with orange the classifiers that can be powered up by a printed Molex \textit{30 mW} battery \cite{} and with blue those that can be power supplied by a printed Blue Spark \textit{3 mW} \cite{}.
It is observed that for an up to 5\% accuracy loss all the classification circuits can be powered-up by printed batteries, while for 1\% only the pendigits classifier exceeds the \textit{30 mW} power threshold.






\begin{figure}[t]
\centering
\begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/scatter_ww_rw.png} 
\end{subfigure}
\begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/cardio_vertebral_scatter.png}  
\end{subfigure}

\begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/scatter_pendigits_seeds.png}  
\end{subfigure}
\caption{True Pareto fronts after synthesis and gate-level simulation showing normalized power consumption Vs accuracy for three standalone approximation techniques and our framework's at 1V. Examined MLP classifiers: (a) White-wine, (b) Red-wine, (c) Cardio (d) Vertebral, (e) Pendigits, (f) Seeds.}
\label{fig:scatter_plots}
\end{figure}


  
\begin{figure}[t]
\centering
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/barplots1.png} 
    %\caption{}
    %\label{SUBFIGURE LABEL 1}
\end{subfigure}
\begin{subfigure}{\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/barplots2.png}  
    %\caption{}
    \label{fig:barplots}
\end{subfigure}


\caption{Area and power evaluation compared to the approximate bespoke approach \cite{} for 1\% accuracy degradation from our baseline \cite{} (Figures \textbf{(a)}, \textbf{(b)}) and the stochastic approach \cite{} for iso-accuracy designs (Figures \textbf{(c)}, \textbf{(d)}).}
\label{fig:barplots}
\end{figure}



\input{Sections/tab_battery}



==> Sections/old_sections/framework_3.tex <==

\section{Co-design for Printed MLPs}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{Sections/Figures/flow.png}
%     \caption{.}
%     \label{fig:flow}
% \end{figure}





% In this section the hardware-driven optimization approaches and the approximate computing techniques that are used in the proposed framework are presented. This framework efficiently combines a set of known approximation techniques to deliver low-area and low-power circuits for MLP classifiers in printed electronics. It enables a five-stage flow that is depicted in Figure \ref{fig:flow} followed by a customized hardware friendly implementation. Each of the framework's stages aims to minimize the design's occupied on-chip area and its power expenses in different aspects. Namely the framework's stages are:
% \begin{itemize}
%     \item A \textbf{Neural Architecture Search (NAS)} to determine the size and the accuracy of the bespoke baseline classifier's network.
%     \item A low-bit \textbf{quantization} to reduce the size of the operands and therefore the area of the bespoke implemented multipliers and adders.
%     \item A \textbf{Structured Pruning} to remove circuit blocks and hardwired connections among neurons.
%     \item \textbf{Weight Clustering} to enable a more aggressive quantization of the model's coefficients and reduce the number of the multipliers.
%     \item \textbf{Voltage Scaling} to reduce the circuit's operating voltage and minimize its power expenses.
% \end{itemize}
This section presents the proposed co-design methodology (Fig.~\ref{fig:framework}) for printed MLP circuits that combines the hardware-efficiency of bespoke circuits with a hardware-aware neural minimization that is dedicated to such customized implementations.
%An abstract overview of this framework is illustrated in Fig.~\ref{fig:framework}.
For the neural minimization we employ a hardware-aware NAS, quantization, unstructured pruning, and weight sharing.
%Then, voltage scaling is applied synergistically to these techniques to boost the power savings.
%Moreover, voltage scaling is also used at the circuit-level to translate any performance gains due to the neural simplification to additional power savings.
Voltage scaling is additionally applied to boost the power savings.
In the remainder of this section we discuss the application of these techniques and emphasize on their expected hardware impact on printed MLPs.
Finally, we describe our area estimator and the flow of our proposed methodology.

\subsection{Bespoke MLP Circuits}\label{sec:bespoke}
In our work, we leverage the efficiency of bespoke implementations and design a fully customized MLP per dataset.
In addition, we exploit the peculiarities governed by integrating the coefficient values in the circuit description to achieve our hardware-aware neural minimization (see Sections~\ref{sec:nas}-\ref{sec:sharing}).
%The peculiarities governed by integrating the coefficient values in the circuit description are then exploited in our hardware-aware neural simplification (see Sections~\ref{sec:nas}-\ref{sec:sharing}).
For example, the area and power of bespoke circuits are highly correlated with the coefficient values~\cite{Armeniakos:DATE2022:axml}.
%Hence, carefully selecting hardware-friendly coefficients will lead to high area and power gains.
% A descriptive case is the zero-cost coefficients.
% Apparently, all the coefficients that are a power-of-two result in a zero-area multiplier since only shifting and wiring is required.
% However, in bespoke circuits, multiplying a 4-bit positive input $A$ (as in our MLPs that use the Relu activation function) by $17$ also induces zero-area overhead since the product is equal to $\{A, A\}$ and requires only concatenation and wiring.

Integrating the coefficients in the description of a MLP will use bespoke multipliers (i.e., area gains from the multiplications) but the accumulation of each neuron's products will still require a conventional (generic) implementation.
Therefore, optimizing the accumulators is mandatory to achieve high area/power efficiency, albeit that the current state-of-the-art~\cite{Armeniakos:DATE2022:axml,Mubarik:MICRO:2020:printedml,Weller:2021:printed_stoch} disregards them in their analysis and does not optimize them. 
Indicatively, as shown in~\cite{Armeniakos:DATE2022:axml} the area of a bespoke multiplier of a positive 4-bit input by $23$ is identical with the area of the respective multiplier by $111$.
Hence, in~\cite{Armeniakos:DATE2022:axml} the coefficients $23$ and $111$ are considered to be cost-equivalent in their optimization.
Though, this is rather the case since $111$ will generate larger products (by at least one bit) and thus a larger conventional accumulator is required.
We reduce the size of the accumulators by constraining the size (Section~\ref{sec:quantization}) and number (Section~\ref{sec:pruning}) of its summands.
Moreover, we instantiate accumulators of bare-minimum precision. 
To achieve this, we run inference on the train dataset and capture the maximum value for each activation. 
Then, we allocate the bare minimum precision for each product (weights are already known) and consequently for each accumulator.



\begin{figure}[t]
    \centering
    \includegraphics[]{Figures/fig1.pdf}
    \caption{Our framework for hardware-efficient printed MLPs. The proposed co-design methodology combines bespoke circuit implementation with a hardware-aware neural minimization that exploits the features of such customized circuits.}
    \label{fig:framework}
     \vspace{-2ex}
\end{figure}


\subsection{Hardware-Aware Neural Architecture Search} \label{sec:nas}
% NAS aims to determine the size of the network and the values of the training hyper-parameters that lead to a model with an acceptable accuracy. In bespoke ML classifiers the network's coefficients are hardwired in the circuit meaning that the number of the model's trainable parameters affect the design's area efficiency. Besides the size of the network, the range of its coefficients can also determine the design's area overhead as well as the efficiency of the weight clustering approximation technique that is enabled in the framework's next stages. Hence a high value of the regularization hyper-parameter alpha is desired at the model's training phase in order to decrease the coefficients variance and increase the possibility of re-appearing values. The latter enables sharing the multipliers' outputs among neurons and leads to a more efficient weight clustering approach as it is discussed in more detail in subsection \ref{}. NAS is performed by training the model until convergence using sckit-learn with pseudo-random 70\%/30\% split for the train and test sets, an adaptive learning rate, one hidden layer and exploring the number of neurons and the value of the regularization parameter alpha. The output of this stage is the smallest network with the highest value of alpha that meets the accuracy criteria as defined in \cite{}.
Given an input dataset, our hardware-aware NAS aims to extract the most area-efficient model that achieves the highest accuracy.
We implement a simplified macro NAS that identifies the MLP architecture and other training hyper-parameters that lead to the highest accuracy.
Among the extracted models, our hardware area estimator (see Section~\ref{sec:estimator}) is used to select the model with the highest area efficiency.
Since our area model expects fixed-point (integer) weights and activations, the precision of the inputs and weights is set to 4 and 8 bits, respectively.
Though, any high-enough value that delivers floating-point accuracy can be used at this point.

For the NAS, Scikit-learn and the randomized parameter optimization with 5-fold cross validation are used.
The input dataset is randomly split to a $70$\%/$30$\% train/test set ratio.
The inputs are normalized to $[0, 1]$.
Since printed circuits are relatively small, only one hidden layer with up to ten neurons is explored.
Limited-memory BFGS, Stochastic Gradient Descent, and Adam are considered for the solver and Relu is used for the activation function due to its hardware efficiency.

\subsection{Low-Bit Quantization for Bespoke MLPs}
\label{sec:quantization}
% In bespoke networks the exact values of the coefficients and the bit representation of the inputs determine the size of the multiplication and adder blocks. Despite small coefficient values can potentially decrease the design's occupied area and minimize its consumed dynamic power by reducing the size of the arithmetic circuits and the number of the wire connections, the exact input values are not known a priori. Hence the size of each bespoke multiplier and adder is determined by the hardwired values of the coefficients and the provisioned bit representation of the inputs. In the proposed framework the impact of a low-bit quantized ReLU activation function alongside with the quantized coefficients in the classifier's accuracy and occupied area is explored. Although, adopting a low-bit representation in the network's input would lead to a more efficient implementation of the bespoke arithmetic circuits, it could also cause bit truncation and increase the induced error. For that reason an arithmetic saturation circuitry block is implemented for the classifier's quantized activation, as it is described in the following subsection \ref{}.

%Precision scaling (or quantization) is one of the most widely used approximation techniques for neural networks~\cite{EfficientAI:2020}.
%since it preserves the regularity of the compute patterns prevalent in ML models.
%For moderate quantization levels the accuracy loss is negligible but for extremely low precisions the accuracy drop might become significant. 
% In addition to the achieved model compression, weights and activations are quantized to low-precision fixed-point (integer) values requiring, thus, simpler arithmetic and more hardware-efficient circuits.
% In conventional silicon systems, the lower the quantization precision the lower the hardware requirements are.
% Though, in most cases the precision of the hardware is predetermined and the networks are mainly quantized to match it. 
%Quantizing the network to lower precision will result in a little additional dynamic power reduction~\cite{Amrouch:NPUthermal:2020} but no additional area gains.

%Precision scaling (or quantization) is one of the most widely used approximation techniques for neural networks~\cite{EfficientAI:2020}.
Quantizing weights and activations to low-precision fixed-point (integer) values leads to simpler arithmetic and more hardware-efficient circuits.
In conventional silicon systems, the lower the quantization precision the lower the hardware requirements are~\cite{ThermalAwareDNN:TC2022}.
In bespoke MLP circuits the impact of quantization is not that straightforward as in silicon systems.
For example, the area of a bespoke multiplier will depend only on the input precision and the weight value and not on the quantization precision for the weights.
In other words, multiplying an input $A$ by $3$ will always require the same area even if 3 or 8 bits are used to represent the weights.
Also consider the above example in which multiplying by $27$ or $111$ results in the same multiplier area.
Hence, exploring the quantization precision for weights could seem irrelevant.
Nevertheless, low-bitwidth weight quantization delivers some valuable benefits that can boost the overall area efficiency. 
Specifically, the smaller the precision for the weights, the more concentrated they will be in a closed squeezed range, increasing the probability for weight sharing (see Section~\ref{sec:sharing}).
Furthermore, all weights will be small, leading to smaller products overall and thus more area-efficient accumulators.

In addition to the weight quantization, we also explore low-bitwidth activation quantization.
Low activation precision delivers high area savings since it directly determines both the multipliers' area and the accumulator's size.
To that end, the MLP inputs are truncated to the required precision while a quantized Relu (QRelu) is used in the hidden layer.
For the weight and bias quantization stochastic rounding is used as i) it mainly delivers higher accuracy~\cite{QKeras} and ii) the values are determined offline during training.
However, the hardware-friendly truncation is used for the activations.
Similarly, for implementation simplicity we use linear quantization.
In fixed-point arithmetic bespoke circuits, QRelu is efficiently implemented since the position of the decimal point is known, saturation can be implemented with a few OR gates, and truncation is used for the trailing bits below the required precision.
An example of our QRelu implementation is shown in Fig.~\ref{fig:qrelu}.
%\red{Fig. XX shows an example of a 4-bit (Q0.4) QRelu with 8-bit input.}
%Nevertheless, implementing a QRelu induces a hardware overhead compared to a simple full-precision Relu but is usually compensated by the savings originating by using low precision activations in the output layer.
%\red{Still our optimization search (see Section~\ref{sec:framework}) will decide whether Relu or a low-precision QRelu will be used.}
%Targeting implementation simplicity we use linear quantization. 
Qkeras~\cite{QKeras} is used to quantize the model and quantization-aware (re-)train (QAT) is performed to improve the accuracy.
Furthermore, in QAT we use L1-regularization forcing weights to small values and consequently more efficient accumulators.

% \begin{figure}[t!]
% \centering
%     \centering
%     \includegraphics[scale=0.25]{Figures/qrelu.pdf} 
% \caption{QRelu}
% \label{fig:qrelu}
% \end{figure}

 \begin{figure}[t!]
 \centering
     \centering
     \includegraphics[]{Figures/qrelu.pdf} 
 \caption{QRelu circuit with Q4.6 input and UQ1.3 output.}
 \label{fig:qrelu}
 \vspace{-2ex}

\end{figure}

\subsection{Unstructured Pruning} \label{sec:pruning}
% Structured and gate-level pruning are design techniques used for decreasing the neuron connections, omitting circuit blocks \ref{} and increasing the performance, area and power gains. In the context of the proposed framework various levels of pruning sparsity are explored as a complementary approach to the quantization of the network's inputs and coefficients that can lead to additional area and energy savings. However, a high pruning sparsity may have a detrimental effect on the network's quality and depending on the network's size, the sparsity and the circuit's timing constraints; \AK{pruning may make the design prone to timing violations as the decrease in the number of neurons is disproportional to the decrease in the height of the typical adder trees.}
Another popular approach to minimize neural networks is pruning.
In conventional systems structured pruning is mainly preferred as it is easier exploited in hardware albeit that unstructured pruning mainly achieves higher sparsity and/or accuracy.
Though, in bespoke printed MLP circuits, unstructured pruning directly translates to hardware savings.
In our work we use low magnitude unstructured pruning~\cite{Pruning}.
By removing a connection (weight) the corresponding multiplier is removed from the circuit.
In addition, fewer products need to be accumulated leading, thus, to a smaller accumulator at the respective neuron.
As a result, significant hardware gains can be obtained from both the multiplication and accumulation operations.
An illustrative example is shown in Fig.~\ref{fig:examples}a.
%However, considering that printed MLPs are rather small (feature a few weights) extremely high sparsity may lead to untolerable accuracy degradation.
%To that end, when training the MLP we use L1 regularization. 

 \begin{figure}[t!]
 \centering
     \centering
     \includegraphics[]{Figures/examples.pdf} 
 \caption{Examples of the hardware impact of (a) pruning and (b) weight sharing on our bespoke MLPs.}
 \label{fig:examples}
  \vspace{-2ex}
\end{figure}

\subsection{Weight Sharing in Bespoke MLPs}\label{sec:sharing}
% Typically, weight clustering and coefficient sharing are compression techniques that have been introduced as possible solutions for minimizing the network's memory footprint \ref{}. Although in bespoke architectures the hardwired coefficients do not have an impact on the model's memory needs; weight clustering can be leveraged for reducing the number of the bespoke implemented multipliers. Specifically, in fully parallel bespoke architectures of MLP classifiers the number of the on-chip multipliers is equal to
% \begin{equation}
% \begin{aligned}
% M= \sum_{i=1}^{N-1}  n_{i} \cdot n_{i+1},
% \end{aligned}
% \end{equation}
% where \textit{N} is the network's number of layers and \textit{n\textsubscript{i}} is the number of neurons of layer \textit{i}. Hence, when the weights of an input neuron share the same value, one multiplier can be implemented and used for propagating its output to all accumulations. Despite this technique can decrease the number of the implemented multipliers, it may also increase the design's power expenses as a few multiplication blocks will need drive larger loads. 

% In the context of the proposed framework the weight clustering methodology that was introduced in 2016 by Han et al. \cite{} is followed. This clustering technique employs a K-means algorithm for grouping the weights of each layer into \textit{K} clusters, where the values of the weights are replaced by the corresponding value of its centroid. In this framework this clustering technique is used alongside the methodologies described in subsection \ref{nas}, \ref{quantization} and \ref{pruning} meaning that the network's coefficients that are generated after this step will be low-bit quantized values that will belong in \textit{K} discrete bins.
Weight sharing is a compression technique that has been introduced as a tentative solution for minimizing the network's memory footprint~\cite{sharing:ICLR2016}.
%However, in the case of printed bespoke MLPs, weight sharing can deliver significant hardware gains.
However, we employ weight sharing to achieve hardware gains.
Assume that in the same layer, weights of different neurons, that are multiplied with the same input, feature the same value.
In that case only one bespoke multiplier needs to be instantiated and its product can be reused in more than one neurons (e.g., Fig.~\ref{fig:examples}b).
As a result, less multipliers are required but the number of summands in each neuron remains the same. 
%However, the load capacitance of that multiplier will increase, potentially affecting the circuit's performance.
When optimizing for area, the EDA synthesis tools auto-detect (sub)expression sharing and if a model exhibits high weight-sharing potential, then area and power efficient implementations are seamlessly obtained.

In our neural minimization, after the MLP is pruned and quantized, we further approximate the model by forcing weight sharing.
To achieve this, we implement a modified version of~\cite{sharing:ICLR2016}.
%First, we freeze the hardware-friendly weights.
%By hardware-friendly we refer to all the weights that the respective bespoke multiplier features zero-area (not only powers-of-two, see Section~\ref{sec:bespoke}).
K-means is used for grouping the non-pruned same-input weights of each layer into \textit{K} clusters and the values of the weights are replaced by the corresponding value of its centroid.
The clustered weights are also frozen and we retrain the MLP to recover the accuracy loss. 

Finally, to additionally increase the probability of multiplier sharing, we split the weights of each neuron into two groups that comprise the positives and negatives ones.
An example of our weight sharing implementation is shown in Fig.~\ref{fig:examples}b.
The absolute value of the weights is used for the bespoke multiplier.
Considering that the inputs are always positive (e.g., due to Relu), the sign of the weight determines the product's sign.
By accumulating separately the products of each group and then subtracting the sums, we obtain the expected result.
The benefit of ``artificially’’ removing the negative weights is twofold.
Firstly, the area of a positive bespoke multiplier is less than the area of the corresponding negative one~\cite{Armeniakos:DATE2022:axml}.
Secondly, the probability for multiplier sharing is theoretically doubled since the possible values for the bespoke multipliers are halved, increasing the possibility of re-appearing values.



\subsection{Voltage Scaling} \label{sec:voltage}
%Decreasing the circuit's operating voltage is the framework's final optimization step and aims to significantly decrease the design's consumed power. Specifically, three operating voltages 0.6V, 0.8V and 1V are examined per design. A decrease in the operating voltage, however, doesn't typically lead to area gains; designs that are generated to operate in low voltages may struggle to meet their timing constraints and therefore larger circuit blocks will be employed for their implementation. The feasibility of this technique depends mainly on the network's size, as in large networks a decrease in the operating voltage may cause timing violations.
Approximating a circuit usually makes it faster~\cite{ThermalAwareDNN:TC2022}.
This delay gain can be leveraged to lower the voltage value and further improve the power-efficiency at the same performance as the exact baseline~\cite{ThermalAwareDNN:TC2022}.
Though, voltage scaling does not deliver any area gains.
In our case, using low-precision operands (input activations and weights) makes the bespoke multipliers smaller since less partial products need to be accumulated.
Moreover, the products are also smaller leading to smaller carry-chains and faster accumulators.
Furthermore, pruning weights removes products, resulting in accumulators of smaller depth and potentially faster.
Leveraging the performance boost due to our neural minimization, we perform a binary search to find the minimum voltage value that satisfies a user’s specified delay constraint.
Hence, additional power savings are achieved without any timing errors due to the voltage drop.
Considering that EGT printed circuits (as in our case) may be operated at only $0.6$V~\cite{Marques:Materials:2019}, a high performance gain from minimizing the network may lead to high additional power gains.

% \subsection{Hardware-Driven RTL Optimizations}
% \label{synthesis}
% The designs that are generated by the proposed framework are optimized based on the aforementioned approximation techniques and synthesized using the Synopsis Design Compiler mapped to the open source Electrolyte Gate Transistor (EGT) technology \cite{}. The Register-Transfer Level (RTL) description of each implemented design is optimized to facilitate the deployment of the described techniques. At first, the network's inputs are scaled in the \((0,1)\) range which decreases their variance and turns them into positive values.

% To enable an effective multiplication sharing approach, the sign of the negative coefficients is reversed, transforming them into their equivalent positives. As a result the range of the network's coefficients is shrinked from \([-w,w]\) to \([0,w]\) where \textit{w} is the maximum appearing value. This approach groups together the negative and positive coefficients, increases the possibility of re-appearing values and leads to the generation of fewer bespoke multipliers. Finally, two accumulations are performed; one for the multiplication products that were produced from the originally positive coefficients and a second one for the originally negatives. The second accumulation is subtracted from the first and the neuron's output that is subsequently fed in the ReLU activation function is produced. 

% In the context of this framework a low-bit quantized ReLU is used as described in subsection \ref{quantization} which may cause an accumulation error due to bit truncation. Hence, a saturation circuit block is synthesized, forcing the value of the ReLU activation function to its maximum quantized value in case of an accumulation overflow.

\subsection{Proposed Bespoke Area Estimator}\label{sec:estimator}
Our introduced area estimator lies at the core of our framework,
abstracting the unique features of bespoke printed MLP circuits and enabling high level exploration of the neural minimization parameters (see Section~\ref{sec:framework}).
%To abstract the unique features of bespoke printed MLP circuits and enable high level exploration of the neural simplification parameters (see Section~\ref{sec:framework}), we propose an area estimator model.
Using our estimator, we can run our hardware-aware neural minimization without requiring circuit synthesis to evaluate each design solution.
Time-efficiency is critical considering the in-situ, on demand, and low-volume fabrication of printed circuits.
%that, unlike silicon-VLSI, might prohibit long-running design and optimization processes.
The main elements that contribute to a printed bespoke MLP’s area are i) the bespoke multipliers, ii) the conventional accumulators, and iii) QRelu of each neuron.
A circuit’s area can be estimated by the sum of the area of its sub-components.
Denoting a MLP as $M$, a neuron as $N$, a weight as $w$, a bespoke multiplier by $w$ as $BM_w$, we express the MLP area as follows:

{\vspace{-\baselineskip}\small
\begin{gather}
\mathrm{AREA}(MLP) = \sum_{\mathclap{\forall N \in M}}{\mathrm{AREA}(N)}, \raisetag{-20pt}\\ \notag
\mathrm{AREA}(N) = \sum_{\mathclap{\substack{\forall w \in N |\\ w\, \text{not shared}}}}{\mathrm{AREA}(BM_w)} \!+\! \mathrm{AREA}(Add) \!+\! \mathrm{AREA}(QRelu)
\label{xo}
\end{gather}
}

$\mathrm{AREA}(BM_w)$:
As aforementioned, the area of a bespoke multiplier depends on the coefficient value and the input precision.
Hence, $\forall w\in [0, 128]$ (we use the absolute values in the circuit description and weights are up to 8 bits) we run an offline process in which we synthesize all the $BM_w$ for all the supported input precisions (see Section~\ref{sec:framework}) and store the area values in a look-up table ($\mathrm{LUT}$).
Hence, if $z$ is the input precision, $\mathrm{LUT}(z,w)$ gives the area of the respective bespoke multiplier.
Each evaluation requires less than a second and all the evaluations are fully parallelizable.
To identify if a weight $w$ is shared or not, we just need to check if it has the same absolute value with any of the same-input weights of the previous neurons of the same layer.

$\mathrm{AREA}(QRelu)$:
QRelu requires only an inverter (INV) and a few AND and OR gates.
The number of the required gates depends only on the QRelu's input and output precision (e.g., Fig.~\ref{fig:qrelu}).
Assume that the input is in the Q$I_i$.$F_i$ format and the output in the UQ$I_r$.$F_r$ one.
Considering that the printed technology library~\cite{Bleier:ISCA:2020:printedmicro} comprises only 2-input OR gates, then:

{\vspace{-0.7\baselineskip}\small
\begin{equation}
\begin{split}
    \mathrm{AREA}(QRelu)=&\mathrm{AREA}(\text{INV})+(I_r+F_r)\cdot\mathrm{AREA}(\text{AND})\\
                         &+max(I_i-I_r-1,0)\cdot\mathrm{AREA}(\text{OR}),
\end{split}
\label{eq:qrelu}
\end{equation}
}

\noindent
where the area of the AND, OR, and INV is constant and obtained directly from the technology library.

$AREA(Add)$: The area of the accumulator depends on the number and precision of the summands (products).
Overall, the area of an accumulator is proportional to the number of the required full-adders.
However, since in bespoke architectures the coefficients are hardwired, the EDA tools will do constant propagation to further optimize the logic.
In addition, the summands (products) are proportional to the weight values.
Hence, we express the area of the accumulator as a linear regression (LR) of the neuron's weights.
For all possible input sizes, we randomly generate $100$ accumulator samples and synthesize them to obtain their area and train our LR model.
We train a LR per input precision.
Each synthesis requires a few seconds and they can run fully in parallel.
Assuming $W$ the list of neuron's weights and $z$ the input precision, the area of the accumulator is estimated by $AREA(Add)=LR_z(W)$.

% We evaluate the accuracy of our area estimator using 1,000 randomly generated printed MLPs.
% The $R^2$ score of our area estimator is $0.75$.
% Most importantly, its Pearson correlation coefficient is $0.89$, i.e., very good linear correlation.
% Hence, our estimator can predict with high confidence if a MLP is more area efficient than another one and guide our optimization search (see Section~\ref{sec:framework}) towards more efficient solutions.

\subsection{Proposed Co-design Framework for Bespoke MLPs }\label{sec:framework}
Our framework (Fig.~\ref{fig:framework}) operates as follows:

\subsubsection{First step}
Using the input dataset and our area estimator, we run our hardware-aware NAS (Section~\ref{sec:nas}).
An MLP that features the highest accuracy and minimum area estimation is extracted. 

\subsubsection{Second step}
The obtained model is pruned (Section~\ref{sec:pruning}) with the target sparsity level and then the weights, activations, and biases are quantized (Section~\ref{sec:quantization}) using the desired precision values.
Then, QAT is executed
%with learning rate $10^{-4}$
to fine-tune the quantized weights.
To identify the optimal value for these hyper parameters, we employ the elitist NSGA-II genetic algorithm from the open-source framework pymoo~\cite{pymoo:2020} to explore the design space and find the solutions that minimize the design objectives of printed bespoke MLPs:

{\small
\begin{equation}\label{eq:opt}
\begin{gathered}
\min_{w,b,r,i,s} \, \mathrm{AccuracyLoss}(MLP_N,c,b,r,i,s)\\
\min_{w,b,r,i,s} \, \mathrm{AreaEstimation}(MLP_N,c,b,r,i,s),
\end{gathered}
\end{equation}
}

\noindent
where $MLP_N$ is the model obtained from NAS, $s$ is the target sparsity level, and $c$, $b$, $r$, and $i$ are respectively the precision levels for the weights, biases, activations of the output layer (i.e., QRelu precision), and input precision.
%If full precision is used for $r$, then Relu is used instead of QRelu.
As in QKeras, the precision levels are in the form ($P$,~$I$) where $P$ specifies the number of bits for the quantization, and $I$ specifies how many bits of $P$ are used for the integer part.
The number of bits ($P$) for $c$ and $b$ is $\leq 8$, for $i$ is $\leq 4$, and for $r$ $\leq 8$.
Finally, the examined sparsity levels are $\leq 50$\% with a $10$\% step. $w$, $b$, $r$, $i$, and $s$ are encoded in the chromosomes' genes.
Each chromosome generates an MLP with a unique set of parameters.
The accuracy of each MLP is evaluated and its hardware efficiency is assessed using our area estimator (Section~\ref{sec:estimator}). The output of our genetic optimization is the Pareto front of the solutions that minimize the optimization objectives~\eqref{eq:opt}. 
\subsubsection{Third step}
We apply our weight sharing (Section~\ref{sec:sharing}) on the MLPs extracted in step 2.
All possible values for the number of clusters ($K$) at each layer are considered.
Though, note that $K$ is well bound by the limited number of weights in the neurons.
Again, our area estimator is used to obtain the new accuracy-estimated area Pareto front.

\subsubsection{Fourth step}
The final step of our framework is to generate the bespoke hardware descriptions (Section~\ref{sec:bespoke}), in Verilog, of the MLPs obtained from the previous step.
The obtained circuits are synthesized at the minimum voltage value that satisfies a user-defined delay constraint (see Section~\ref{sec:voltage}). 
%It is assumed that the delay constraint can be met at $1$V.

\noindent
Then, circuit simulation and power analysis with switching activity annotation are performed to obtain the circuit's power and verify that its accuracy meets the software (QKeras) extracted one.
Finally, among the analyzed designs the power-accuracy and/or area-accuracy Pareto front is the output of our framework.
Note that at this stage, the area is not estimated but it is calculated from the EDA tools.

% The illustration depicted in Figure \ref{fig:framework} shows the flow of the proposed framework. Starting from NAS where an optimal in terms of size and inference accuracy model is trained followed by the optimizations that quantize and prune the network. At this stage a multi-objective optimization problem is defined to determine the bit representation of the quantized parameters and the network's pruning sparsity. This problem is formulated as it it shown below and aims to find the hardware parameters that minimize the network's inference error and the design's occupied on-chip area.

% \begin{equation}
% \begin{aligned}
% \min_{w,b,r,i,s} \quad & 1-accuracy(w,b,r,i,s)\\
% \min_{w,b,r,i} \quad & area(w,b,r,i) \\
% \textrm{s.t.} \ &
%   2 \leq w\leq 7 \text{ , w: weights}    \\
%  & 2 \leq b\leq 7 \text{, b: biases}   \\
%  & 2 \leq i\leq 4 \text{, i: input}    \\
%  & 3 \leq r\leq 8 \text{, r: ReLU}    \\
%  & 10\% \leq s\leq 50\% \text{, s: sparsity}    \\
% \end{aligned}
% \end{equation}

% To estimate the design's area a Look-Up Table (LUT) is created where the area overhead of one multiplier at an operating voltage of 1V is stored for input and coefficient sizes ranging from one to 7 and one to 8 bits respectively. Based on the generated LUT a linear predictive model is trained to estimate the overall area that will be occupied by the network's multipliers and adders combined.

% The proposed framework employs the elitist NSGA-II \cite{} genetic algorithm from the open-source framework pymoo \cite{} to explore the design space and find the solutions that minimize the problem's objectives. The bit-width of the network's coefficients, inputs and the pruning sparsity are encoded in the chromosomes' genes. Each chromosome generates a network with a unique set of parameters.

% To enable an effective quantization and pruning scheme of the pre-trained network's parameters, a quantization-aware
% (QA) retraining and an inference evaluation is performed for all the generated networks using the open source framework QKeras \cite{}. The learning rate in the QA retraining is set to \(1 \cdot e ^{-4}\) to fine-tune the quantized network's coefficients, the Adam optimizer is used  the number of epochs is determined offline and ranges between one to 15 depending on the examined network.

% The output of the genetic optimization is the Pareto front of the solutions that minimize the optimization objectives. At the following stage, the weight clustering technique is enabled. At this optimization step the coefficients of the generated Pareto optimal solutions are grouped in a range of two to \(M\) clusters using the methodology that was described in subsection \ref{clustering}. At the end of this process \(n + n \cdot M \) RTL descriptions using the implementation methodology that was described in subsection \ref{synthesis} are produced, where \(n\) is the number of the Paretos.

% Noted, that the aforementioned automated process leads to the generation of an estimated Pareto front due to the approximate calculation of the design's occupied area. The estimated Pareto solutions are synthesized for the operating voltages described in subsection \ref{voltage} and the true Paretos of the hardware feasible solutions are extracted. 






==> Sections/old_sections/introduction_1.tex <==

\section{Introduction}

The exponential increase in the production of consumer goods such as agricultural, healthcare, and packaged products has made imperative the need of enabling smart services for an efficient time and cost management of the supply chain.
Services for the item identification and quality monitoring of the fast moving consumer goods (FMCG) require the deployment of smart devices on the packaging of the products~\cite{Bleier:ISCA:2020:printedmicro}.
%Despite conventional silicon-based semiconductors are used for the design of smart systems their lack of flexibility, stretchability and their manufacturing cost make the deployment of those devices prohibitive.
%On the other hand, printed electronics (PE) devices are typically built on paper and plastic substrates and 
Printed electronics (PEs)
form a promising solution for the implementation of such systems due to their low cost, high flexibility, and conformity~\cite{Bleier:ISCA:2020:printedmicro}.

Such features could never be met by silicon VLSI systems.
Printing technologies often rely on mask-less, portable, and additive manufacturing methods which can greatly reduce costs and production timelines. 
PEs require low-cost equipment and refer to the fabrication technology that relies on printing processes, such as jet, screen or gravure printing~\cite{Bleier:ISCA:2020:printedmicro}.
In such printed technologies, functional solution-based materials are additively printed to form active (transistors, diodes) and passive (resistors, capacitors, interconnects) components for fully-printed electronics. However, this comes at much higher feature sizes (micrometers), lower device counts (1000s), and lower frequencies (few Hz to$\sim$KHz) compared to silicon VLSI.
%PE technologies are broadly categorized to i) additive manufacturing that involves only deposition steps and ii) subtractive process that involves a series deposition and etching processes, similar to silicon-based process.
%PE technologies are broadly categorized to i) additive manufacturing that involves only deposition steps and ii) subtractive manufacturing that involves a series of additive (deposition) and subtractive (etching) processes, similar to silicon-based process.
%PEs feature several prevalent limitations such as the large feature sizes and low integration density that
%\AK{Those limitations} may lead to unacceptable hardware overheads as well as high device latencies.
%PE and silicon VLSI systems cannot compete each other but are complementary technologies.
%PE will never achieve silicon-based integration density, performance, etc.,  while the latter will never realize ultra-low cost and flexible computing systems.
%Despite the benefits of PE, their large feature sizes may lead to a unsustainable area and power overheads, making the realization of complex designs infeasible. 

Still, PEs attract vast research and industrial interest and printed computing systems have been successfully fabricated.
In 2020 Ozer et al.~\cite{Ozer:Nature:2020} fabricated a natively flexible processing engine for an odour recognition application.
In 2021 ARM fabricated an extreme low cost 32-bit processor with TFT (Thin Film Transistor) technology on a flexible plastic substrate for deployment on everyday objects~\cite{ARM:2021}.
In 2022, PragmatIC Semiconductor~\cite{ISCA2022} fabricated and tested multiple 4 and 8-bit flexible microprocessors optimized for high yield.
%designed a processing engine on a flexible substrate and evaluated its functionality by executing an odor recognition algorithm
%while the same year Weller et al.~\cite{Weller:ASPDAC:2020:neuron} printed an artificial neuron on EGFET technology.

The large feature sizes in PEs render the design of complex circuits, e.g., for Machine Learning (ML), extremely challenging and even unrealistic in many cases~\cite{Armeniakos:DATE2022:axml,Weller:2021:printed_stoch, Mubarik:MICRO:2020:printedml}.
%The first attempt for printed ML classification is reported in~\cite{Mubarik:MICRO:2020:printedml}.
Leveraging the extremely low fabrication and non-recursive engineering (NRE) costs of PEs that allow on-demand and in-situ printing,~\cite{Mubarik:MICRO:2020:printedml} proposed the design of bespoke printed ML circuits.
In such circuits the degree of customization is so high that each circuit is fully tailored to a specific ML model. 
%This level of customized implementations enables area- and power- efficient designs~\cite{Ozer2019Bespoke,Bleier:ISCA:2020:printedmicro} that are mostly infeasible in lithography-based silicon technologies, mainly due to their high fabrication and NRE costs~\cite{Bleier:ISCA:2020:printedmicro}.
The latter enables extremely optimized designs~\cite{Ozer2019Bespoke,Bleier:ISCA:2020:printedmicro} that are mostly infeasible in lithography-based silicon technologies, mainly due to their high fabrication and NRE costs~\cite{Bleier:ISCA:2020:printedmicro}.
Bespoke ML classifiers are designed in~\cite{Mubarik:MICRO:2020:printedml} by hardwiring the model’s coefficients in the circuit implementation itself.
Despite the high gains,~\cite{Mubarik:MICRO:2020:printedml} deduced that circuits such as Multilayer Perceptrons (MLPs) are very complex and focused on simple ML circuits (e.g., Decision Trees).
Alternative computing paradigms such as approximate~\cite{Honglan:AxSurvey:2020} and stochastic~\cite{Liu:TCASI:2021} computing could form promising solutions to mitigate the elevated hardware overheads of printed MLPs.
Approximate printed MLPs are designed in~\cite{Armeniakos:DATE2022:axml} achieving high but inadequate area and power savings.
In~\cite{Weller:2021:printed_stoch} very area-efficient stochastic printed MLPs are designed that feature, however, significant accuracy loss.

ML arguably forms a perfect match with approximate computing due to many factors.
In our work, we exploit this relation and combine it with the unmatched hardware-efficiency of bespoke implementations~\cite{Mubarik:MICRO:2020:printedml,Ozer2019Bespoke,Bleier:ISCA:2020:printedmicro} targeting battery-powered printed MLPs.
Our holistic neural minimization framework is built upon hardware-aware Neural Architecture Search (NAS), pruning, quantization, and weight sharing, while at the hardware level voltage scaling is also used.
In our framework we exploit the unique features and irregularities of bespoke circuits and tailor these techniques to printed MLPs.
Through our bespoke MLP area estimator we jointly apply these techniques in a printed-driven manner since the implication of model-specific bespoke hardware affects all optimization steps of such methods.
Although such techniques are also used in Deep Neural Network (DNN), the optimization objectives are fundamentally different.
Our goal is to squeeze hardware costs (area/power) to meet physical constraints, such as available batteries and harvesters, end-product area requirements etc., while still getting decent accuracy.
Considering the limited device counts and large feature sizes in PEs, our primary objective regards even the feasibility of such systems.
This is essentially different from DNN optimization for generic, model agnostic silicon-based devices (e.g., GPUs, TPUs) that even in the case of FPGAs does not offer the customization degree available in printed circuits.

%To that end, we propose a systematic co-design methodology that exploits the peculiarities of bespoke circuits and implements an automated hardware-aware neural simplification dedicated for such fully-customized MLP circuits.
%Our holistic neural minimization framework is built upon hardware-aware Neural Architecture Search (NAS), pruning, quantization, and weight sharing, while at the hardware level voltage scaling is also used.
The MLPs generated by our framework exhibit $4.1$x less area than the state-of-the-art exact (un-minimized) baseline~\cite{Mubarik:MICRO:2020:printedml} for no accuracy loss while for only $5$\% loss we enable battery-powered operation of all the examined MLPs.
%that feature up to $15$ neurons and $130$ parameters.

\noindent
\textbf{The novel contributions of our work are as follows:}
\begin{enumerate}[topsep=0pt,leftmargin=*]
\item We propose an efficient area estimator that abstracts the unique features of fully customized printed MLPs, enabling thus their high-level optimization.

\item This is the first automated hardware-aware neural minimization framework for printed MLPs.

\item Our co-design methodology enables, for the first time, the realization of high-accuracy battery-powered complex  MLPs in PEs.

%with up to $15$ neurons and $130$ parameters.


\end{enumerate}


==> Sections/old_sections/references.tex <==
\begin{thebibliography}{00}



\end{thebibliography}

==> Sections/old_sections/tab_battery.tex <==
  %\begin{table}[t]
  %\centering
  %\caption{}
 % \vspace{-.1in}
 % \footnotesize
%  \resizebox{\columnwidth}{!}{
      %\begin{tabular}{c|c|c|c|c}
      %\hline
      %\textbf{Classifier} & \textbf{Accuracy} & %\textbf{Voltage (V)} & \textbf{Area %(cm\textsuperscript{2})} & \textbf{Power (mW)} \\ %\hline
     % \rowcolor{molex}
     % WhiteWine & 0.53 & 0.6 & 12.4 & 12 \\
     % \rowcolor{molex}
     % WhiteWine & 0.51 & 0.6 & 3 & 4 \\ \hline
     % \rowcolor{bluespark}
     % RedWine & 0.55 & 0.6 & 1 & 1 \\
     % \rowcolor{bluespark}
     % RedWine & 0.51 & 0.6 & 0.7 & 0.6 \\ \hline
     % \rowcolor{molex}
     % Cardio & 0.87 & 0.6 & 5.5 & 5.3 \\
     % \rowcolor{molex}
     % Cardio & 0.83 & 0.6 & 2.9 & 3.1 \\ \hline
    %  \rowcolor{molex}
    %  Vertebral & 0.86 & 0.6 & 3.3 & 3.3 \\ \hline
      
      %Vertebral & 0.86 & 0.6 & 3.3 & 3.3 \\ \hline
    %  Pendigits & 0.93 & 0.8 & 22.9 & 40.6 \\
    %  \rowcolor{molex}
    %  Pendigits & 0.89 & 0.8 & 14  & 26.8 \\ \hline
   %   \rowcolor{molex}
   %   Seeds & 0.93 & 0.6 & 4.5 & 4.5 \\
   %   \rowcolor{bluespark}
   %   Seeds & 0.88 & 0.6 & 1.6 & 2 \\ \hline
    
   %   \end{tabular}
%     }
  %  \label{tab:table_platforms}
 %   \vspace{-.1in}
 % \end{table}

   \begin{table}[t]
  \centering
  \caption{Hardware analysis of the printed MLPs produced by our framework for 1\% and 5\% accuracy loss thresholds.}
 \label{tab:battery}
  \footnotesize
  \setlength\tabcolsep{4pt}
  \begin{threeparttable}
      \begin{tabular}{c|c|c|c|c|c|c|c}
      \hline
      \textbf{Classifier} &
      \textbf{Acc.} &
      \makecell{\textbf{Acc.} \\ \textbf{Loss\tnote{\tiny *}}} &
      \makecell{\textbf{Area} \\ (\textbf{cm}$^\mathbf{2}$)} &
      \makecell{\textbf{Area} \\ \textbf{Gain\tnote{\tiny *}}} &
      \makecell{\textbf{Power} \\ \textbf{(mW)}} &
      \makecell{\textbf{Power} \\ \textbf{Gain\tnote{\tiny *}}} &
      \makecell{\textbf{Voltage} \\ \textbf{(V)}} \\ \hline
      
  \rowcolor{zinergy}
      WhiteWine\tnote{\tiny +} & 0.53 & 0.01 & 12.4 & 2.5x &12 & 8.2x & 0.60 \\
 \rowcolor{zinergy}
      WhiteWine & 0.51 & 0.05 & 3.0 & 10.4x & 4.0 & 24.6x  & 0.60 \\ \hline
 \rowcolor{harvester}
      RedWine & 0.55 & 0.01 & 1.0 & 17.6x & 1.0 & 53.3x & 0.60  \\
 \rowcolor{harvester}
      RedWine & 0.51 & 0.05 & 0.6 & 29.3x & 0.7 & 76.1x & 0.60  \\ \hline
\rowcolor{zinergy}
      Cardio & 0.87 & 0.01 & 5.5 & 6x & 5.3 & 18.3x & 0.60 \\
\rowcolor{bluespark}
      Cardio & 0.83 & 0.05 & 2.9 & 11.5x  & 3.1 & 31.3x & 0.60  \\ \hline
\rowcolor{zinergy}
      Vertebral & 0.86 & 0.00 & 3.3 & 2.6x & 3.3 & 12.6x & 0.60 \\ \hline
      
      %Vertebral & 0.86 & 0.6 & 3.3 & 3.3 \\ \hline
      Pendigits & 0.93 & 0.01 & 22.9 & 2.92x & 40.6 & 5.24x & 0.80 \\
\rowcolor{molex}
      Pendigits & 0.89 & 0.05 & 14  & 4.7x  & 23 & 9.2x & 0.74\\ \hline
\rowcolor{zinergy}
      Seeds & 0.93 & 0.01 & 4.5 & 2.2x & 4.5 & 10x & 0.60 \\
\rowcolor{harvester}
      Seeds & 0.88 & 0.05 & 1.6 & 6.1x  & 2.0 & 22.5x & 0.60 \\ \hline
    
      \end{tabular}
      \begin{tablenotes}\footnotesize
\item[] $^*$ With respect to the respective baseline MLP~\cite{Mubarik:MICRO:2020:printedml}.
\item[] $^+$ Colors denote a printed battery that can power each MLP.\\
Orange: $30$mW, light blue: $15$mW, dark blue: $3$mW, green: harvester.

\vspace{-4pt}
\end{tablenotes}
\end{threeparttable}
\vspace{-12pt}
  \end{table}

